Meta-theorems for Graph Polynomials

In this paper I survey the sources of inspiration for my own and co-authored work in trying to develop a general theory of graph polynomials. I concentrate on meta-theorems, i.e., theorem which depend only on the form infinite classes of graph polynomials are defined in some formalism, and not on the actual meaning of the particular definitions.

==> NMA-short.tex <==
\section{Introduction}

\subsection{One, two, many graph polynomials}
In my paper \cite{makowsky2008zoo}
I set myself the goal of developping a general theory of graph polynomials.
The paper was written after my realization, together with Boris Zilber, that there are many more naturally occurring
graph polynomials
than are treated in the literature, see my papers \cite{makowsky2023got} and  
Kotek, Makowsky and Zilber \cite{ar:KotekMakowskyZilber08}. 
In analogy to the matching polynomial or the independence polynomial, which use the number of $k$-matchings or 
$k$-independent sets as coefficients of a generating function, 
one can use
the number of configurations on $k$ vertices (or edges) given by a description in some logical formalism
as coefficients of a generating function. 
The domination polynomial is a good example, but there are no limits in creating such graph polynomials.
We also noticed that counting the number of conditional colorings treated in the literature
gives graph polynomials in the number of colors which I named later Harary polynomials, see Section \ref{se:harary}.
Earlier attempts to define large classes of graph polynomials go back to Farrell \cite{ar:Farrell79a}.

The discovery of the abundance of naturally defined graph polynomials led some mathematicians in search of a topic to 
define somehow an arbitrarily defined new graph polynomial, say $F(G;x)$, and investigate it
by dealing with one or more of the following questions:
\begin{enumerate}[(i)]
\item
Compute $F(G_n;x)$ for selected graph families $G_n: n \in \NN$;
\item
Find $F(G;x)$-unique graphs;
\item
Interpret $F(G;a)$ for selected values $a \in \ZZ$ in terms of graph theoretic properties of $G$; 
\item
Interpret the polynomials $F(G_n;x)$ for certain sequences of graphs $G_n$;
\item
Compare the distinguishing power of $F(G;x)$ to the distinguishing power of some other graph polynomial $F'(G;x)$.
\item
Is $F(G;x)$ in some sense ``equivalent'' to some previously studied graph polynomial $F_0(G;x)$?
\item
Where are the roots of $F(G;x)$ located?
\end{enumerate}
The same questions can also be asked for multivariate polynomials.

Some of the more exciting papers in graph polynomials have dealt with such questions, but more recently
I have seen many papers where the choice of $F(G;x)$ is badly, if at all, motivated, and only a few answers to
these questions were given.


\subsection{Meta-theorems}
The purpose of this paper is to show what I had, and still have, in mind 
by a ``general theory of graph polynomialsa'' 
%in the first formulation of my aim 
in \cite{makowsky2008zoo}. 

Let me first give a (admittedly trivial) example of a meta-theorem.

Assume we want to show that a certain graph property, say triangle-free, is hereditary (closed under induced subgraphs).§
We can show this directly in the framework of graphs. But we can also observe that triangle-free can be expressed
by a universal first order formula $\pi$:
$$
\phi :
\forall u,v ( E(u,v) \leftrightarrow E(v,u)) \wedge
\forall u,v,w ( 
\neg E(u,v) \vee
\neg E(v,w)) \vee
\neg E(w,u))
).
$$
Now it is easy to show that any graph property expressible by a universal first order formula $\psi$
is hereditary. 
This is a {\em meta-theorem} since it uses only the fact that $\psi$ is a universal first order formula,
irrespective of the particular meaning of $\psi$.
If we allow infinite graphs as well, the well known {\L}o\'s-Tarski  Theorem asserts that the 
converse is true as well: 
\begin{theorem}[{\L}o\'s-Tarski Theorem]
Let $\cA$ be a class of
(possible infinite) graphs axiamatizable by a set of first order sentences $\Sigma_{\cA}$.
Then $\cA$ is hereditary if and only if $\Sigma_{\cA}$ is logically equivalent to a set of universal first order sentences.
%is is axiomatizable by a set of universal sentences in $\FOL$
\end{theorem}
If restricted to finite structures, Tait \cite{Tait1959} showed that it is wrong even if $\Sigma_{\cA}$ is finite.

There is another way of formulating a meta-theorem for hereditary classes of graphs.
A class of finite graphs  $\cA$ is hereditary if and only if it can be characterized by a (possibly infinite) set 
$\Forb_ {\cA}$ of forbidden induced subgraphs. There the mere existence of $\Forb_ {\cA}$, irrespective
of the elements of $\Forb_ {\cA}$ guarantees that $\cA$ is hereditary.
This can also be formulated in infinitary logic by a universal formula of $\mathcal{L}_{\infty, \omega}$, see
\cite{rosen1995preservation}.
Applied to graph polynomials rather than graph properties
we should look for theorems of the following type:
\begin{tcolorbox}
Let $\cF$ be a class of graph polynomials 
and $\cC$ a class of graphs, both
defined in some logical formalism. 
Then for every $G \in \cC$ and $F(G;\bar{x}) \in \cF$
the graph polynomial $F(G;\bar{x})$ exhibits a characteristic behaviour or property
irrespective of the  particular meaning of the definition of $\cF$ and $\cC$.
\end{tcolorbox}
This can be viewed  as a meta-theorem if it only depends on the form of how $\cF$
and $\cC$ are defined, and not on the particular choice of these definitions.
%I consider such theorems as {\em meta-theorems} because 
%the properties of the graph polynomials derived only depend on the propertis of $\cF$ and $\cC$.

An early, possibly the earliest, meta-theorem in graph theory is the Specker-Blatter Theorem from 1981, 
\cite{blatter1981lenombre,specker1990application,fischer2011application}.

\begin{theorem}[Specker-Blatter Theorem]
Let $\phi$ is a formula in Monadic Second Order Logic in the language of graphs.
Let $S_{\phi}(n)$ be number of binary relation $E \subset [n]^2$ such that
graph $G = ([n], E)$ satisfies $\phi$.
Then sequence
$S_{\phi}^m(n) = S_{\phi}(n) \pmod{m}$
is ultmately periodic with
$$
S_{\phi}^m(n) = S_{\phi}^m(n+p_{m,\phi})
$$
for all $n \geq q_{m,\phi}$.
\end{theorem}
We consider this a meta-theorem, since ultimate periodicity is a consequence of the syntactic form of $\phi$ only
(but the values $p_{m,\phi}, q_{m,\phi}$ depend on $m$ and $\phi$).
At the time of publication in 1981 (and till 2000) this theorem was widely unnoticed.
For its history and recent developments, see \cite{fischer2024extensions}.


\subsection{Towards a general theory of graph polynomials}
Since  the publication of \cite{makowsky2008zoo} my collaborators and I have achieved some progress in developng the 
modest beginnings of such a general theory.
The following sections we give examples and discuss such meta-theorems in detail.

In Section \ref{se:recursion} we discuss theorems inspired by results about the Tutte polynomial
and Tutte-Grothendieck invariants ($\TG$-invariants) and similar theorems.
More generally, we outline our results from \cite{godlin2012graph} about unwinding recursive definition of
graph polynomials.

In Section \ref{se:complexity} we review general theorems about the complexity of evaluating
graph polynomials. This includes Fixed Parameter Tractable ($\FPT$) cases for graph classes of bounded
width (tree-width, clique-width, rank-width, etc), and dichotomy theorems for graph polynomials
arising from partition functions.


In Section \ref{se:unimodality} we discuss general theorems about real-rooted graph polynomials
and graph polynomials where the coefficients satisfy concavity conditions.
The special cases of graph polynomials where the coefficients are unimodal is here of special interest.

In Section \ref{se:harary} we review some results about Harary polynomials.

In Section \ref{se:weakly} we discuss a conjecture by Bollob\'as, Pebody and Riordan which states that
the Tutte polynomial is almost complete. A graph polynomial $F(G;\bar{x})$ is almost complete
if almost all graphs are $F$-unique.
We contrast this to graph polynomials $F(G;\bar{x})$ being weakly distinguishing if almost
all graphs $G$ have a $F$-mate and prove a meta-theorem about weakly distinguishing graph polynomials.

In Section{se:semantic} we briefly introduce and discuss the distinction between syntactic and semantic statements 
about (families of) graph polynomials.

Finally, in Section \ref{se:conclu} we draw conclusions and suggest some further research along the lines described
in this paper.

\subsection*{Acknowledgements}
My PhD students of the last 25 years, Udi Rotics \cite{phd:Rotics}, Ilia Averbouch \cite{phd:Averbouch}, 
Tomer Kotek \cite{phd:Kotek} and Vsevolod Rakita \cite{phd:Rakita}, contributed
much to these developments. So did my co-authors, Benny Godlin, Orli Herscovici, Emilia Katz, Elena Ravve 
and Ruixue Zhang.
Markus Bl\"aser, 
Holger Dell, 
Andrew Goodall,
Miki Hermann and
Steve Noble joined me in studying the complexity of graph polynomials.
I would like to thank Graham Farr, Kerri Morgan, Vsevolod Rakita, Elena Ravve and Peter Tittmann for reading and commenting
on earlier drafts of this paper. Their observations and sugeestions were all incorporated into the final version.

\subsection*{The Matrix Institute}
Two events of the Matrix Institute had great impact on my work described in this paper:
the Tutte Centenary Retreat in December 2017 and the Workshop on Uniqueness and Discernement in Graph Polynomials
in October 2023. 
I would like to thank the Matrix Institute and the organizers of these meetings for their fruitful initiatives:
Graham Farr, Dillon Mayhew, Kerri Morgan, James Oxley and Gordon Royle in 2017, and
Jo Ellis-Monaghan, Iain Moffat, Kerri Morgan and Graham Farr in 2023.



%Since then I have achieved some progress in developng the modest beginnings of such a general theory.
%The purpose of this paper is to show what I had in mind. 



